FairNet: A Measurement Framework for Traffic Discrimination Detection on the Internet

Network neutrality is related to the non-discriminatory treatment of packets on the Internet. Any deliberate discrimination of traffic of one application while favoring others violates the principle of neutrality. Many countries have enforced laws against such discrimination. To enforce such laws, one requires tools to detect any net neutrality violations. However, detecting such violations is challenging as it is hard to separate any degradation in quality due to natural network effects and selective degradation. Also, legitimate traffic management and deliberate discrimination methods can be technically the same, making it further challenging to distinguish them. We developed an end-to-end measurement framework named FairNet to detect discrimination of traffic. It compares the performance of similar services. Our focus is on HTTPS streaming services which constitute a predominant portion of the Internet traffic. The effect of confounding factors (congestion, traffic management policy, dynamic rate adaptation) is made `similar' on the test services to ensure a fair comparison. FairNet framework uses a ``replay server'' and user-client that exchanges correctly identifiable traffic streams over the Internet. The Server Name Indication (SNI) field in the TLS handshake, which goes in plaintext, ensures that the traffic from the replay server appears to network middle-boxes as that coming from its actual server. We validated that appropriate SNIs results in the correct classification of services using a commercial traffic shaper. FairNet uses two novel algorithms based on application-level throughput and connection status to detect traffic discrimination. We also validated the methodology's effectiveness by collecting network logs through mobile apps over the live Internet and analyzing them.

==> intro__Manjesh_Kumar_Hanawal_s_conflicted_copy_2021-10-12_.tex <==
As commercial activities surge on the Internet, the expectations on the Internet have gradually emerged towards `guaranteed service' rather than  'best-efforts' service for which it was originally designed. Internet Service Providers (ISPs) are using various means to maintain high quality for services that are more commercially viable and degrade quality for other commercially less viable services or that generated from the competitors. There are growing cases of unjustified service-specific throttling \cite{wehe_res_2019}, site-blocking that are recently reported. Also, there are regulatory provisions for ISPs to perform reasonable traffic management that could impact the performance of specific applications but increase the overall experience for users \cite{eu_allows_throttling,rjio-site-blocking}. Under such a complex ecosystem, regulators opt for net neutrality (NN) as a guideline to distinguish malicious from lawful network management practices. To enforce any neutrality laws, one has to have a mechanism to identify any deliberated discrimination. This work proposes a method to detect any deliberate traffic discrimination (TD) or NN violations on the Internet.
%Network neutrality is related to the ``non-discriminated" treatment of the same type of traffic (video, audio, file transfer) on the Internet irrespective of their origin and destination. Though many countries have laws enforcing neutrality, they also allow discrimination of the traffic for ``reasonable" network management. 


Our focus in this work is on the audio and video media streaming services. These services occupy over $66\%$ of market share with $50\%$ of services using 4K HD videos (requiring around 25 Mbps speed) \cite{int_study}. To main high quality of service (QoS) and user experience, media streaming services services use Dynamic Adaptive Streaming over HTTP (DASH) as one of methods used by media streaming services for maintaining required QoS. These schemes are proprietary and could differ across the content providers. Moreover, the services now use HTTPS protocol which provides the end-to-end encryption of the services and makes it difficult for the ISPs to look int payload and classify the traffic. 


Many tools have been developed for detecting traffic differentiation \cite{nn_survey_2018}. 
Most of the tools use client-server architecture where services that need to be checked for discrimination are replayed from a dedicated server referred to as a `common server'—the contents from services of interest are copied from the original server and stored in the common server (CS). Thus CS acts as a proxy of the original server. To check whether a service is subjected to discrimination, the client accesses that service from the CS and compares the QoS it receives against reference traffic. The basic hypothesis for detection is that traffic accessed from the CS (target flow) is treated from the network middleboxes as though it is originated from the original server and will be subjected to intended discrimination, whereas the reference flow will not be classified by the middleboxes and will evade the discrimination. Thus, comparing the quality of service of the two flows will reveal any discrimination of the service of interest. 
%The existing tools suffer many limitation when used to detect discrimination of HTTPS traffic. The primary issue is the target traffic that is generated from the replay server may not be treated in the same way as they treat the traffic from the original serer and will be incorrectly classified. This is due to the following reasons: 1) application servers use  Dynamic Adaptive Streaming over HTTP (DASH) to give best user experience to the end users. This may not be captured by the replay server. 2) the existing tools use port 80 for replay of encrypted traffic which will be treated by default as un-encrypted traffic and may not detect any useful signatures. 3) The reference traffic used for comparisons with target traffic may evade the classification, but may be treated belong to a non-classified service class. This service class may be treated differently than the service of interest and thus comparisons of performance of target and reference traffic may not lead to correct conclusions.

The existing tools suffer many limitations when used to detect discrimination of HTTPS traffic. The primary issue is that the target traffic generated from the CS may not be treated in the same way as they treat the traffic from the original server and lead to incorrect classification of services. Mis-classification could be due to the following reasons: 1) CS may not capture the application server's DASH mechanism. 2) the existing tools use port $80$ to replay encrypted traffic, which will be treated by default as un-encrypted traffic and may not detect any useful signatures. 3) The reference traffic used for comparisons with target traffic may evade the traffic classification but may be treated as some default class and receive a different QoS from the intended service. Thus comparisons of target and reference traffic performance may not lead to correct conclusions.

To overcome these issues, we develop a new framework for measurement named Fairnet. Fairnet also uses a client-server architecture. The server hosts all the services of interest taken from original servers (by sniffing or direct downloading) and replays them on demand. Fairnet overcomes the limitation of the exiting tools as follows: 1) The CS uses a custom DASH so that the traffic is adapted to the actual network environment making the replay traffic appear more genuine. Customized DASH at the CS avoids bandwidth overshoot above available bandwidth and ensures similar data transmission rates for all services under consideration. 2) Fairnet sends Server Name Indication (SNI) filed in the TLS handshake appropriate for the service. SNI filed goes unencrypted in the TLS handshake phase and can be read by the middle-boxes. 3) Instead of comparing target traffic with a reference traffic, we compare the performance of traffic of service with traffic of another service of a similar type. For example, to check if YouTube is being discriminated, we compare it to another service like Netflix or Hotstar that has similar service requirements.  

Fairnet measurement framework is based on sound principles. Network middle-boxes look for plain-text information in addition to the other signature they could extract from the encrypted payload, e.g., packet size, inter-arrival time. Server Name Indication (SNI) field in the TLS handshake is one such field that goes in plain text and is thus reliably used by the network middle-boxes to classify traffic of different services \cite{trcl_survey}. If one notices any performance degradation of a specific traffic stream (say YouTube), it is hard to pinpoint the actual cause of the degradation. Instead, we can compare the performances of similar traffic streams (say YouTube vs Prime Video or YouTube vs Netflix) to measure the relative performances where deliberate discrimination could become apparent. Thus, it is important to compare services requiring similar QoS for the comparisons to result in meaningful conclusions. Comparison of traffics requiring similar QoS requirements to detect TD is also one of the recommendations by the Body of European Regulators for Electronic Communications (BEREC) \cite{berec_1101} to detect deliberation discrimination on the Internet. 

% FairNet measurement framework uses the customised DASH at server side to avoid bandwidth overshoot above available bandwidth and to ensure similar data transmission rates for all services under consideration. 

% middle-boxes will apply the policy of classifying uncrypted traffic on this and may not get any sig un-encrypted traffic and trea  
% used by the application servers and strong encryption from the HTTPS protocol removes any unique signatures from the traffic. 


% Network middle boxed look for files plain-text information in addition to the other signature they could extract from the encrypted payload, e.g., packet size, inter-arrival time. Server Name Indication (SNI) field in the TLS handshake is one such field that goes in plain text and is thus reliably used by the network middle-boxes to classify traffic of different services \cite{trcl_survey}. 

% Our focus in this work is on the media streaming services. These services occupy over 66$\%$ of market share with $50\%$ of services using 4K HD videos (requiring around 25 Mbps speed) \cite{int_study}. DASH is one of methods used by media streaming services for maintaining required QoS. These schemes are proprietary and could differ across the content providers. FairNet measurement framework uses the customised DASH at server side to avoid bandwidth overshoot above available bandwidth and to ensure similar data transmission rates for all services under consideration. 

% If one notices any performance degradation of a specific traffic stream (say YouTube), it is hard to pinpoint the actual cause of the degradation. Instead, we can compare the performances of similar traffic streams (say Prime Video, Netflix, YouTube) to measure the relative performances. For the comparisons to result in meaningful conclusions, one should compare services requiring similar quality of services. This is inline with BEREC's \cite{berec_1101} guidelines.

Our traffic discrimination (TD) detection algorithm compares the throughput performance of a target service with that of another service requiring similar QoS. Use of common the CS, DASH, simultaneous access of serices, and comparison of similar types of services ensures that the effect of confounding factors on QoS (delay, jitters, throughput) will be largely similar. Thus any major variation in the performance of two traffic streams can be attributed to deliberate TD. 
%Further, setting the correct SNI parameters always the HTTPS traffic is correctly classified by the network middle-boxes. We verify that our replay traffic is correctly classified as intended traffic using a commercial traffic shaper. Our contributions can be classifed as follows:
% Any major variations in quality of service in the Fairnet frame work . 

% Thus it reflects the network congestion conditions experienced by each service. The data rates of services thus varies if they are routed through different congestion paths. Such source data rate variations are considered as throughput variations while performing TD detection.

% All the traffic simultaneously streaming between the ``common server" and FairNet user-client is likely to  on the Internet, and hence the effect of confounding factors on QoS (delay, jitters, throughput) will be similar. A similar data transmission scheme such as DASH on the server controls the data rate of transmissions of all the streams identically. 

%The normalisation of network TMPs, congestion effects and source rate (i.e. DASH) ensures that all traffic flows under considerations experience similar network effect at the end-user. Consequently, the following sentences summarise the contributions of this paper.
\begin{itemize}
\item We provide a mechanism to make the replay traffic from the CS appear as though it is generated from the orginal server to the middle-boxes. FairNet uses the original service's SNI value in the initial TLS handshake message. Due to this parameter setting, the network middle-boxes correctly classify traffic replayed from the CS. We verify using a commercial traffic shaper that all our replayed traffic are classified as intended services. 
\item We ensure that the effect of network confounding factors is normalized across all services simultaneously accessed from the CS. FairNet exchanges traffic between dedicated client and server simultaneously using a customized DASH. This normalizes the network effects such as congestion, network TMPs, and server-side data transmission mechanisms. Thus all services under test are expected to experience similar network effects, and any measured performance can be used for direct comparison to detect any deliberate discrimination.     
\item FairNet uses the novel TD detection algorithm (refer Sec. \ref{sec:tddetectalgo}) based on downloaded file size, connection breaks, and received throughput performance. It directly compares the average throughput within a time slot across services while considering the performance similar to that of the service under test to avoid false detection.
\item Based the Fairnet measurment framework, we develop an Android and iOS mobile which are available on Google Playstore and Apple AppStore. Using the app we collect the measurment traces from the Internet (refer Sec.\ref{sec:Deployment}). 
\item We systematically analyze the traces and discuss discrimination of various services in the Internet (refer Sec. \ref{sec:Deployment}). 
\end{itemize}


==> methodology.tex <==
Our methodology for detecting traffic discrimination uses performance comparison of traffic streams of similar types. This is a delicate task as the effect of Internet-borne, legitimate traffic management, and dynamic adaptive streaming techniques on QoS of traffic are hard to distinguish from each other.  We refer to them as performance confounding factors. We next discuss the problem that each of these types of performance degradation creates for generating comparable performance metric to detect traffic discrimination. 
\begin{itemize}
	\item {Internet borne:} The notion of similar network conditions is hypothetical because the Internet is free to route packets from the server through any physical route considering the best-effort delivery policy. The difference in the physical path between source and destination also contributes briefly by making different streams experience different congestion levels.
	\item {Legitimate traffic management:} The different types of services with varying QoS requirements undergo different traffic management techniques. It is applied by ISP mainly for the overall efficiency of the network through load balancing while providing an acceptable level of performance to all services. As a consequence, different types of services over the Internet experience inherently different performances. 
	\item {Adaptive streaming:} The data transferred by the multimedia streaming server is a function of many parameters like multimedia block length, compression techniques, inter-fetch time of data blocks. These parameters vary across streaming services depending on the adaptive streaming protocol used by the services, and hence the performance measured across different services could vary. 
\end{itemize}

Thus it is hard to conclude whether any observed poor QoS is due to deliberate discrimination or natural congestion in the network. Our measurement framework ensures that the aspects mentioned above affect all the traffic streams in the same manner, imparting the same level of performance degradation. If there is deliberate degradation of the quality of a traffic stream, only that stream's quality further degrades and could be identified by performance comparison. 

\begin{figure}[htbp]
	\centerline{\includegraphics[scale=.4]{./Figs/perf_convert}}
	\caption{Comparable performance metric after unifying contributing parameters}
	%\Description{Comparable performance metric after unifying contributing parameters}
	\label{fig:perf_convert}
\end{figure}

Fig. \ref{fig:perf_convert} shows throughput for four streaming services, named A, B, C, D. Left figure shows the effect of confounding factors on throughput when they are accessed from the original server and the right figure shown when their effect are removed/equalized by our measurement framework (right figure). In the left figure, the total height of each bar (consisting of the colored and grayed portion) shows throughput for each streaming service as governed by the transmission strategy (DASH in case of streaming services) of their servers.
The colored portion (other than grey) shows the throughput experienced at the client-side. The grey portion is the throughput lost in the network -- the upper part of the grayed portion shows the throughput lost due to network congestion and the lower grayed portion shows that lost due to network traffic management. Note that the server of each stream could be sending the traffic at different rates with their own proprietary DASH and that received by user-clients depend on the different levels of degradation the streams experience in the networks. The white portion in the throughput performance bar of service D shows throughput lost due to deliberate degradation. Identifying this discrimination of stream D just by comparing the throughout experienced at the user-client will be misleading due to non-uniformity in the transmission rates at the source and network effects.

The plot on the right-hand side shows the throughput performance when all performance confounding factors are aligned to the same level for all services (server rates, congestion, traffic management). In this case, any deliberate degradation over the degradation from the confounding factors can be contrasted by comparing the throughput performance at the client and thus can be detected.
